Graph-Theoretic Approach to Quantum Error Correction

We investigate a novel class of quantum error correcting codes to correct errors on both qubits and higher-state quantum systems represented as qudits. These codes arise from an original graph-theoretic representation of sets of quantum errors. In this new framework, we represent the algebraic conditions for error correction in terms of edge avoidance between graphs providing a visual representation of the interplay between errors and error correcting codes. Most importantly, this framework supports the development of quantum codes that correct against a predetermined set of errors, in contrast to current methods. A heuristic algorithm is presented, providing steps to develop codes that correct against an arbitrary noisy channel. We benchmark the correction capability of reflexive stabilizer codes for the case of single qubit errors by comparison to existing stabilizer codes that are widely used. In addition, we present two instances of optimal encodings: an optimal encoding for fully correlated noise which achieves a higher encoding rate than previously known, and a minimal encoding for single qudit errors on a four-state system.

==> app_proof.tex <==
\section{Proof of Theorem~\ref{cayley thm}}\label{proofs}

\begin{appthm}{\ref{cayley thm}}%\label{cayley thm}
Let $C$ be a linear subspace of $\mathbb{F}_d^n$ where $d=p^m$. The LUC graph $G(C)$ has exactly $d^{n-\op{dim}(C)}$ number of connected components, each of which is complete. Moreover, the connected component which contains $\overline{0}$ is exactly $C$.
\end{appthm}
\begin{proof}
Due to linearity of $\mathbb{F}_d^n$, it is enough to show the connected component, $H$, containing $\overline{0}$ is complete and contains exactly the elements from $C$. It is clear that $\overline{0}$ is connected to exactly those $c\in C$. Moreover, if $b\notin C$, then $b-a\notin C$ for any $a\in C$. Hence the connected component containing $\overline{0}$ contains exactly the elements of $C$. Lastly, by linearity of $C$, if $a,\ b\in C$, then $b-a\in C$ and thus $(a,b)\in E\Big(G(C)\Big)$. Thus $H$ is complete. 
\end{proof}

% The following theorem shows the connection between LUC graphs and reflexive quantum stabilizer codes.

% \begin{thm}\label{graph correct}
% Let $d=p^m$ for some prime $p$, $G(C)$ be a LUC, and $C_2\subset C^\perp_1\subset\mathbb{F}_d^n$ a linear subspace, then $R^C_{C_1}$ can correct any error from the set $\mathscr{E}$, if 
% \begin{equation*}
% % \left.\Big\{E_1\inv E_2\, \right|\  E_1,E_2\in\mathscr{E}\Big\}
% D(\mathscr{E})\subseteq\left\{\omega^\kappa D_{a,b}\;\Big|\;(a,b)\nin E\Big(G(C)\Big),\,a\nin C_1,\,\kappa\in\{0,...,p-1\}\right\}
% \end{equation*}
% and 
% \begin{equation*}
% \mathscr{A}_\mathscr{E}\cap C_1=\{0\}. 
% %\left.\Big\{E_1\inv E_2\, \right|\  E_1,E_2\in\mathscr{E},\,\kappa\in\{0,...,p-1\}\Big\}
% \end{equation*}
% \end{thm}
% \begin{proof}
% \RV{maybe something like... we wait for this proof until later??}Let $\mathscr{E}$ be an error set such that $R^X_{C_1,C_2}$ can correct $\mathscr{E}$. Next, let $E:=\omega^\kappa D_{a,b}\in D(\mathscr{E})$, thus $E\nin S^\perp$ for the $S$, the stabilizer of $R^X_{C_1,C_2}$ by Theorem \ref{errorcorrecting}, and thus by Corollary \ref{stables} we have $a-b\nin C_1$ and $a\nin C_2^\perp$ as desired. Again by Corollary \ref{stables} if $\omega^k D_{a,a}\in\mathscr{E}^2$ and $a\nin C_2^\perp$ then $\omega^k D_{a,b}\nin S^\perp$ and hence by Theorem \ref{errorcorrecting} our code can correct as desired.
% \end{proof}

==> correction.tex <==
\section{Error correction}\label{error correction}
Before we examine the error correction capabilities of reflexive codes we cover a basic property of stabilizer codes. Given a commutative subgroup $S\subset\mathcal{E}_n$  then clearly a quantum stabilizer code associated to $S$ can protect from error in $S$. 
For a quantum code to be able to protect from any error in an error set $\mathscr{E}\subset\mathcal{E}_n$, it is necessary and sufficient \cite{errortheory,mixed} for any two code words $|c_1\ran$, $|c_2\ran$ in our quantum code with $\lan c_1|c_2\ran=0$, and any two errors $E_1,E_2\in\mathscr{E}$, we have
\begin{equation*}
\begin{split}
\lan c_1|E_1\inv E_2|c_2\ran&=0,\\
\lan c_1|E_1\inv E_2|c_1\ran&=\lan c_2|E_1\inv E_2|c_2\ran.
\end{split}
\end{equation*}
It is of note that we will always assume $\mathbb{1}\in\mathscr{E}$ as one should always protect from no errors occuring. 

\begin{defn}\label{E2}
Given any two errors from an error set $E_1,E_2\in\mathscr{E}$, we will refer to $E_1\inv E_2$ as a \textbf{conjugate error} of $\mathscr{E}$. Furthermore, we will denote the set of conjugate errors of $\mathscr{E}$ by 
\begin{equation}%\label{E2}
\mathscr{E}^2:= \left.\Big\{E_1\inv E_2\, \right|\  E_1,E_2\in\mathscr{E}\Big\}.
\end{equation}
Furthermore, we define the \textbf{avoidance set} as 

\begin{equation}\label{avoidance}
\mathcal{A}_{\mathscr{E}}:=\left.\Big\{a\in\mathbb{F}_d^n\, \right|\ \omega^\kappa D_{a,a}\in \mathscr{E}^2\text{ for some }\kappa\Big\}.
\end{equation}
\end{defn}

To find codes later we will use the power of our parametric treatment of these error operators. Specifically, for any subgroup $S\subset\mathcal{E}_n$ such that $\mathcal{Z}\subset S$, we associate a linear subspace $\mathcal{L}_S$ of $\mathbb{F}_d^{2n}$ given by   
\begin{equation}\label{ls}
    \mathcal{L}_S=\left\{(\overline{a},\overline{b})\in\mathbb{F}_d^{2n}\,\left|\,D_{\overline{a},\overline{b}}\in S\right.\right\}.
\end{equation} 
It remains only to define a joint eigenspace of $S$; i.e.\ we need only find a basis $\{\overline{v}_i\,:\, i\in\{1,...,\op{dim}(\mathcal{L}_S)\}\}$ for $\mathcal{L}_S$, and then choose eigenvalues for $D_{\overline{v}_i}$, denote these as $\lambda_{\overline{v}_i}$. Thus it follows from Equation \ref{eqcomm} that the errors of $\mathcal{E}_n$ permute the eigenspaces of $\lambda_{\overline{v}_i}$. 


The following theorem follows identically to that in \cite[Theorem 1]{ortho} and \cite[Theorem 3]{nonbinary}. We include it for later reference. 

\RV{possibly moved to prelims}
\begin{thm}\label{errorcorrecting}
Let $S$ be a commutative subgroup of $\mathcal{E}_n$ which contains the center, i.e.\ $\mathcal{Z}\subset S$, and let $S^\perp$ be the subgroup such that $\mathcal{L}_{S^\perp}=\mathcal{L}_S^\perp$ with respect to the inner product from 
Equation \ref{star}. 
% Further, let $E_1,E_2\in\mathscr{E}\subset\mathcal{E}_n$ for an error set $\mathscr{E}$ such that either $E_1\inv E_2\in S$ or $E_1\inv E_2\nin S^\perp$. Then any stabilizer code for $S$ is an error-correcting code which will correct any error $E\in\mathscr{E}$.
Further, let $\mathscr{E}\subset\mathcal{E}_n$ be an error set.  Then any stabilizer code for $S$ is an error-correcting code which will correct any error from $\mathscr{E}$ if and only if every conjugate error $E\in\mathscr{E}^2$ satisfies either $E\in S$ or $E\nin S^\perp$. 
\end{thm}

Next we specialize to the case of reflexive codes. 

\subsection{Reflexive codes}
Now we begin exploring the basic error correction capabilities for these new codes. 
\begin{defn}\label{detgroup}
Given a linear subspace $C\subset\mathbb{F}_d^n$ we define the \textbf{non-detection group}, denoted $S_C^\perp$ as the subgroup of $\mathcal{E}_n$ generated by %the following set,
\begin{equation}\label{nondet}
% \left.\Big\{\omega^\kappa\mathbb{1}\,\right|\,\kappa\in\{1,...,p-1\} \Big\}\cup\left\{\left.D_{\overline{a},\overline{a}+\overline{b}}\,\right|\,\overline{a}\in\mathbb{F}_d^n,\;\; \overline{b}\in C^\perp\right\}
S_{C}^\perp:=\left\lan\omega^\kappa\mathbb{1},\,D_{\overline{a},\overline{a}+\overline{b}}\,:\,\overline{a}\in\mathbb{F}_d^n,\;\;\overline{b}\in C^\perp,\ \kappa\in\{0,1,\ldots,p-1\}\right\ran.
\end{equation}
where $C^\perp$ is the orthogonal space with respect to the inner product in Equation \ref{inner}. 
It is easy to check that this satisfies $\mathcal{L}_{S^\perp}=\mathcal{L}_S^\perp$ from the previous theorem, where $\mathcal{L}_S$ is given in Equation~\eqref{ls}.
\end{defn}

An immediate consequence of Theorem \ref{errorcorrecting} and Theorem \ref{refcode} is the following.
\begin{cor}\label{correctref}
Let $C\subset\mathbb{F}_d^n$ be a linear subspace, and   $\mathscr{E}\subset\mathcal{E}_n$ be an error set. Then $R_{C^\perp}$ is an error-correcting code which will correct any single error from $\mathscr{E}$ if and only if, for any conjugate error $E\in\mathscr{E}^2$, either $E\in S_C$ or $E\nin S_C^\perp$.
\end{cor}

% \subsection{Reflexive codes}
We now dive into the  error correction capabilities and limitations of a Reflexive QECC $R_C$. We begin 
with general qudit errors and provide a complete description of the possible error sets which $R_C$ can correct. 
\begin{defn}
For an error set $\mathscr{E}\subset\mathcal{E}_n$ we define the \textbf{difference set} of $\mathscr{E}$ as the set 
% \begin{equation*}
% D(\mathscr{E}):=\left.\Big\{\overline{a}-\overline{b}\,\right|\,\exists E_1,E_2\in\mathscr{E},\;\; E_1\inv E_2=\omega^\kappa D_{\overline{a},\overline{b}}\Big\}
% \end{equation*}
\begin{equation*}
D(\mathscr{E}):=\left.\Big\{\overline{b}-\overline{a}\,\right|\,\exists\kappa,\;\;\omega^\kappa D_{\overline{a},\overline{b}}\in \mathscr{E}^2\Big\}
\end{equation*}
\end{defn}

% \begin{lem}\label{diffset lemma}
% Let $C$ be a non-trivial linear subset of $ \mathbb{F}_d^n$ and $\mathscr{E}\subset\mathcal{E}_n$ be an error set. Then 
% \end{lem}

\begin{thm}\label{referrors}
Let $C\subseteq\mathbb{F}_d^n$ be a non-trivial linear subset. Then $R_C$ can correct any error of an error set $\mathscr{E}\subset\mathcal{E}_n$ if and only if 
\begin{equation*}
D(\mathscr{E})\cap C=\{\overline{0}\}\;\;\text{and}\;\; 
\mathcal{A}_{\mathscr{E}}\subseteq C^\perp. 
\end{equation*}
% \begin{equation*}
% \left.\Big\{ \overline{a}\,\right|\,\exists E_1,E_2\in\mathscr{E},\;\; E_1\inv E_2=\omega^\kappa D_{\overline{a},\overline{a}}\Big\}\subseteq  C^\perp.
% \end{equation*}
% and
% \begin{equation*}
% \left.\Big\{ \overline{a}\,\right|\,\exists \kappa,\;\; \omega^\kappa D_{\overline{a},\overline{a}}\in\mathscr{E}^2\Big\}\subseteq  C^\perp.
% \end{equation*}

%\DW{The second line means that the reflexive elements of the conjugate error set are contained in $S_{C^\perp}^\perp$. }
\end{thm}
\begin{proof}
% Let $E\in\mathscr{E}^2$ be a conjugate error of the error set $\mathscr{E}$.
By Theorem~\ref{errorcorrecting} (or Corollary~\ref{correctref}), $R_C$ can correct any error from $\mathscr{E}$ if and only if, for any conjugate error $E\in\mathscr{E}^2$, either $E\in S_{C^\perp}$ or $E\nin S_{C^\perp}^\perp$. 
We see that $\omega^\kappa D_{\overline{b},\overline{c}}\in S^\perp_{C^\perp}$ if and only if $\overline{b}-\overline{c}\in C$, since for any $\overline{a}\in C^\perp$ the following must hold
\begin{equation*}
\begin{split}
(\overline{a},\overline{a})\star(\overline{b},\overline{c})&=\lan\overline{a},\overline{c}\ran-\lan\overline{a},\overline{b}\ran=\lan\overline{a},\overline{c}-\overline{b}\ran=0.
\end{split}
\end{equation*}
Hence, $\omega^\kappa D_{\overline{b},\overline{c}}\in S^\perp_{C^\perp}\setminus S_{C^\perp}$ if and only if $\overline{b}-\overline{c}\in C$ and $\overline{b}\neq\overline{c}$, and thus our theorem follows.
%and suppose the two conditions from the theorem statement hold. Then, by assumption, if $E$ is of the form $\omega^\kappa D_{\overline{a},\overline{a}}$, then $\overline{a}\in C^\perp$. Thus $E\in S_{C^\perp}$. If instead $E$ is of the form $\omega^\kappa D_{\overline{a},\overline{b}}$, for $\overline{a}\neq \overline{b}$, then $\overline{b}-\overline{a}\nin C$, and thus $E\nin S_{C^\perp}^\perp$. Hence, $R_C$ can correct any error from $\mathscr{E}$ by Corollary~\ref{correctref}.

%Let $E\in\mathscr{E}^2$ be a conjugate error of the error set $\mathscr{E}$, and suppose the two conditions from the theorem statement hold. Then, by assumption, if $E$ is of the form $\omega^\kappa D_{\overline{a},\overline{a}}$, then $\overline{a}\in C^\perp$. Thus $E\in S_{C^\perp}$. If instead $E$ is of the form $\omega^\kappa D_{\overline{a},\overline{b}}$, for $\overline{a}\neq \overline{b}$, then $\overline{b}-\overline{a}\nin C$, and thus $E\nin S_{C^\perp}^\perp$. Hence, $R_C$ can correct any error from $\mathscr{E}$ by Corollary~\ref{correctref}.

%Next, suppose $R_C$ can correct any error from $\mathscr{E}$. \DW{Then, if we have a result about $\mathscr{E}$ being a subset of $S_{C^\perp}^\perp$ we would be done. We don't, so we need to use the definition. What follows is the earlier proof.}

% Using Theorems \ref{errorcorrecting} and \ref{refcode} we see that $\omega^\kappa D_{\overline{b},\overline{c}}\in S^\perp_{C^\perp}$ if and only if $\overline{b}-\overline{c}\in C$, since for any $\overline{a}\in C^\perp$ the following must hold
% \begin{equation*}
% \begin{split}
% (\overline{a},\overline{a})\star(\overline{b},\overline{c})&=\lan\overline{a},\overline{c}\ran-\lan\overline{a},\overline{b}\ran=\lan\overline{a},\overline{c}-\overline{b}\ran=0.
% \end{split}
% \end{equation*}
% Hence, $\omega^\kappa D_{\overline{b},\overline{c}}\in S^\perp_{C^\perp}\setminus S_{C^\perp}$ if and only if $\overline{b}-\overline{c}\in C$ and $\overline{b}\neq\overline{c}$, and thus our theorem follows.
\end{proof}
Now we consider some special cases of the above theorem. 

\begin{defn}\label{singleerror}
In lieu of the second condition of Theorem~\ref{referrors}, we aim to construct the largest error set so that $D(\mathscr{E})$ has nothing of the form $\omega^\kappa D_{a,a}$. 
Let $P\subseteq\{1,...,n\}$, we first denote
\begin{equation*}
\mathcal{P}=\op{Span}_{\mathbb{F}_d}\left.\Big(e_i\,\right|i\in P\Big)
\end{equation*}
where $e_i$ is the $i^{\text{th}}$ standard basis element of $\mathbb{F}_d^n$. Now define the \textbf{$\mathbf{t}$-qudit error set for $\mathbf{P}$} as:
\begin{equation*}
% \mathscr{N}_t(P):=\mathscr{N}_t^Z(P)\cup \mathscr{N}_t^X(P)=\left.\Big\{D_{\overline{0},\overline{a}}\,\right|\,w(\overline{a})\leq t,\;\;\overline{a}\in \mathcal{P}\Big\}\cup\left.\Big\{D_{\overline{a},\overline{0}}\,\right|\,w(\overline{a})\leq t,\;\;\overline{a}\nin \mathcal{P}\Big\}
\mathscr{N}_t(P):=\left.\Big\{D_{\overline{a},\overline{b}}\,\right|\,w(\overline{a})+w(\overline{b})\leq t,\;\;\overline{a}\in \mathcal{P},\;\;\overline{b}\nin \mathcal{P}\Big\}
\end{equation*}
where $w(\overline{a})$ is the number of non-zero entries in $\overline{a}$. 
\end{defn}
% \begin{defn}\label{singleerror}
% Let $P\subseteq\{1,...,n\}$, we define the single qudit error set for $P$ as:
% \begin{equation*}
% \mathscr{N}_1(P):=\left.\Big\{D_{\overline{0},ae_i}\,\right|\,a\in\mathbb{F}_d^*,\;\;i\in P\Big\}\cup\left.\Big\{D_{ae_i,\overline{0}}\,\right|\,a\in\mathbb{F}_d^*,\;\;i\nin P\Big\}
% \end{equation*}
% where $e_i$ is the $i^{\text{th}}$ standard basis element of $\mathbb{F}_d^n$ and $\overline{0}$ is the vector of all zeros.
% \end{defn}
\begin{rem}
One quickly notes that $\mathscr{N}_t(\emptyset)$ %=\mathscr{N}_t^X(\emptyset)$
consists of all $t$ single-qudit flip errors, and $\mathscr{N}_t(\{1,\ldots,n\})$ %=\mathscr{N}_t^Z(\{1,\ldots,n\})$ 
consists of all $t$ single-qudit phase errors. 
In general, $P$ specifies the expected locations of phase errors, allowing for flip errors on the remaining qudits. 
\end{rem}

% \begin{rem}\label{cor rem}
% Here we describe the set $\mathscr{N}^2_t(P):=(\mathscr{N}_t(P))^2$ as in Equation~\eqref{E2}. The results follow from the application of Equations~\eqref{Dab inv} and \eqref{Dab linear}. %If $E_1,\ E_2\in \mathscr{N}_t^Z(P)$, then $E_1\inv E_2=D_{\overline{0},\overline{b}-\overline{a}}$ for some $\overline{a},\ \overline{b}\in \mathcal{P}$. Similarly, if $E_1,\ E_2\in \mathscr{N}_t^X(P)$, then $E_1\inv E_2=D_{\overline{b}-\overline{a},\overline{0}}$ for some $\overline{a},\ \overline{b}\notin \mathcal{P}$. If $E_1\in \mathscr{N}_t^Z(P)$ and $E_2\in \mathscr{N}_t^X(P)$, then $E_1\inv E_2=\omega^{\lan\overline{a},\overline{b}\ran}D_{-\overline{a},\overline{b}}$. Similarly, if $E_1\in \mathscr{N}_t^X(P)$ and $E_2\in \mathscr{N}_t^Z(P)$, then $E_1\inv E_2=\omega^{\lan\overline{a},\overline{b}\ran}D_{\overline{a},-\overline{b}}$. 
% If $E_1=D_{a,b}$, $E_2=D_{c,d}\in \mathscr{N}_t(P)$, then $E_1\inv E_2=\omega^{\lan b,c\ran} D_{c-a,d-b}$, where $c-a\in\mathcal{P}$ and $d-b\nin\mathcal{P}$ such that $w(\overline{c}-\overline{a})$, $w(\overline{d}-\overline{b}) \leq 2t$. Every conjugate error $E\in \mathscr{N}^2_t(P)$ is of this form. 
% \end{rem}

\begin{lem}\label{nt lemma}
Let $C\subset\mathbb{F}_d^n$ be a non-trivial linear subspace, and $P\subseteq\{1,\ldots,n\}$. Then the avoidance set of $\mathscr{N}_t(P)$ is trivial; i.e.\  \[%\left.\Big\{ \overline{a}\,\right|\,\exists \kappa,\;\; \omega^\kappa D_{\overline{a},\overline{a}}\in\mathscr{N}_t^2(P)\Big\}
\mathcal{A}_{\mathscr{N}_t(P)}=\{\overline{0}\}.\] 
\end{lem}
\begin{proof}
The results follow from the application of Equations~\eqref{Dab inv} and \eqref{Dab linear}. If $E_1=D_{a,b}$, $E_2=D_{c,d}\in \mathscr{N}_t(P)$, then $E_1\inv E_2=\omega^{\lan b,c\ran} D_{c-a,d-b}$, where $c-a\in\mathcal{P}$ and $d-b\nin\mathcal{P}$ such that $w(\overline{c}-\overline{a}) + w(\overline{d}-\overline{b}) \leq 2t$. Every conjugate error $E\in \mathscr{N}^2_t(P)$ is of this form. The result follows. 
\end{proof}

\begin{cor}\label{nt}
Let $C\subset\mathbb{F}_d^n$ be a non-trivial linear subspace, and let $\mathscr{E}\subseteq \mathcal{E}_n$ be an error set such that 
\[%\left.\Big\{ \overline{a}\,\right|\,\exists \kappa,\;\; \omega^\kappa D_{\overline{a},\overline{a}}\in\mathscr{E}^2\Big\}
\mathcal{A}_{\mathscr{E}}=\{\overline{0}\}.\]  Then $R_C$ can correct any error of $\mathscr{E}$  if and only if
% \begin{equation*}
% \left.\Big\{\overline{a}\in\mathbb{F}_d^n\,\right|\,w(\overline{a})\leq 2t \Big\}\cap C=\left\{\overline{0}\right\}
% \end{equation*}
\begin{equation*}
D(\mathscr{E})\cap C=\left\{\overline{0}\right\}
\end{equation*}
In particular, this result holds for the error set $\mathscr{N}_{t}(P)$ for every $P\subseteq\{1,\ldots,n\}$.
\end{cor}
\begin{proof}
By assumption, the second condition of Theorem~\ref{referrors} is trivially satisfied. The result follows. 
\end{proof}




We introduce a final bit of terminology. 
\begin{defn}
For a linear subspace $C\subset\mathbb{F}_d^n$ we define the \textbf{weight of $\mathbf{C}$} as 
\begin{equation*}
\op{wt}(C)=\op{min}\left.\Big\{w(c)\,\right|\,c\in C\setminus\{\overline{0}\}\Big\}
\end{equation*}
where $w(c)$ is the number of non-zero entries of $c$.
\end{defn}

\begin{lem}\label{nt size}
Let $C\subset\mathbb{F}_d^n$ be a non-trivial linear subspace, and let $\mathscr{N}_{t}(P)$ be the error set for some $P\subseteq\{1,\ldots,n\}$ as defined in Definition~\ref{singleerror}. Then $R_C$ can correct any $\left\lfloor\frac{\op{wt}(C)-1}{2}\right\rfloor$ single-qudit errors from the set $\mathscr{N}_t(P)$.
\end{lem}

Our next example illustrates Lemma~\ref{nt size} on a small code. 

\begin{ex}
Consider the 2-dimensional code, $C\subset\mathbb{F}_3^2$, consisting of the following vectors
\begin{equation*}
00,11,22.
\end{equation*}
Following Equation \ref{3ref}, we can embed one qudit ($d=3$) into two qudits as 
\begin{equation*}
\begin{split}
|0\ran&\mapsto |\Psi_{00}\ran=\frac{1}{3}\Big(|00\ran+\omega|01\ran+|02\ran+\omega|10\ran+\omega^2|11\ran+\omega|12\ran+|20\ran+\omega|21\ran+|22\ran\Big)\\
|1\ran&\mapsto |\Psi_{11}\ran=\frac{1}{3}\Big(|00\ran+|01\ran+\omega|02\ran+|10\ran+|11\ran+\omega|12\ran+\omega|20\ran+\omega|21\ran+\omega^2|22\ran\Big)\\
|2\ran&\mapsto |\Psi_{22}\ran=\frac{1}{3}\Big(\omega^2|00\ran+\omega|01\ran+\omega|02\ran+\omega|10\ran+|11\ran+|12\ran+\omega|20\ran+|21\ran+|22\ran\Big)
\end{split}
\end{equation*}
By Lemma~\ref{nt size} this code can correct the errors of $\mathscr{N}_1(P)$ for any $P\subset\{1,2\}$. However, as we show in Corollary~\ref{bad cor}, this code cannot correct from an arbitrary single qudit error. 
\end{ex}



Next, we show that no reflexive stabilizer code can correct all single qudit errors. This is the largest limitation of the code. However, in the Subsection~\ref{extensions}, we show that the code extensions given in Subsection \ref{ext} greatly improve the error correction capabilities. 
Regardless, these codes have merit in their own right, as demonstrated in Section \ref{extensions}, where we show that reflexive codes are optimal when channel noise is given by $\mathscr{N}_t(P)$. 
% Now we present the largest limitation of the code $R_C$.
\begin{cor}\label{bad cor}
For all non-trivial linear subspaces $C\subset\mathbb{F}_d^n$, $R_C$ cannot correct all single qudit errors simultaneously.
\end{cor}
\begin{proof}
For the sake of contradiction, assume one can find a $C\subset\mathbb{F}_d^n$ such that $R_C$ can correct all single qudit errors simultaneously. Denoting by $\mathscr{E}_f$ the set containing all single qudit errors, there exists, for all $e_i$ in the standard basis of $\mathbb{F}_d^n$,  $E\in\mathscr{E}_f^2$ such that $E=\omega^\kappa D_{e_i,e_i}$ for some $\kappa\in\{1,\ldots,p-1\}$. Hence, by Theorem \ref{referrors}, we have that $\mathbb{F}_d^n= C^\perp$ and hence $C=\{\overline{0}\}$ a contradiction.
\end{proof}

 At first, this result begs the question, ``Why study reflexive codes at all?", but conventional wisdom rarely holds when studying quantum mechanics. In what follows, we will show that the framework of reflexive stabilizer codes provides a straightforward algorithm for correcting a set of typical \textit{correlated} errors, allowing for better transmission rates in this scenario. Furthermore, quantum error correct codes that correct single qudit errors already exist. \cite{ortho,perfect,nonbinary}


\subsection{Extensions of reflexive codes}\label{extensions}

We built $\mathcal{N}_t(P)$ to keep the phase and flip errors on different qudits. $C_1$ corrects these types of errors. The extension / subcode by $C_2$ helps tackle the same qudit (phase-flip) errors. By lowering $k$ we should be able to fix more errors. The min means a possibly smaller number of errors are guaranteed to be correctable, but we are able to correct from a larger class of errors. 

\begin{thm}\label{error ext}
Let $C_2\subset C_1\subset\mathbb{F}_d^n$ be linear subspaces, then the codes $R^X_{C_1,C_2}$ and $R^Z_{C_1,C_2}$ can both correct up to $t$ single-qudit flip or phase errors where
\begin{equation*}
t=\op{min}\left\{\left\lfloor\frac{\op{wt}(C_1)-1}{2}\right\rfloor,\op{wt}\left(C_2^\perp\setminus C_1\right)-1\right\}.
\end{equation*}
\end{thm}
\begin{proof}
We show the case for $R^Z_{C_1,C_2}$. The other follows similarly. 
%From Corollary \ref{nt} this code can correct any $\left\lfloor\frac{\op{wt}(C_1)-1}{2}\right\rfloor$-qudit error except $E_1,E_2$ such that $E_1\inv E_2=\omega^\kappa D_{\overline{a},\overline{a}}$ for some $\kappa\in\{0,\ldots,p-1\}$ and $\overline{a}\in \mathbb{F}_d^n$. Hence,
From Remark~\ref{nt size}, our code can correct up to $\left\lfloor\frac{\op{wt}(C_1)-1}{2}\right\rfloor$-qudit errors of any form except $\omega^\kappa D_{\overline{a},\overline{a}}$. 

On the other hand, any error of the form $\omega^\kappa D_{\overline{a},\overline{a}}$ as in $S^\perp$ Corollary \ref{stables} exactly when $\overline{a}\in C_2^\perp$. To see this, recall from Theorem~\ref{stable}, that $R^Z_{C_1,C_2}$ is generated by $S_{C_1^\perp}$ and $\left.\Big\{D_{\overline{0},c}\,\right|\,c\in C_2\Big\}$. Then, we see that for any $c\in C_2$ $D_{\overline{0},c}\in S$ and hence
\begin{equation*}
0=(\overline{a},\overline{a})\star(\overline{0},c)=\lan\overline{a},c\ran
\end{equation*}
Hence $\overline{a}\in C_2^\perp$. Furthermore, some requirement from the definition gives us that  $w(\overline{a})\leq \op{wt}\left(C_2^\perp\setminus C_1\right)-1$, we see that $R^Z_{C_1,C_2}$ can correct up to $\op{wt}\left(C_2^\perp\setminus C_1\right)-1$ errors of this form. 



% To see this, note that for the stabilizer $S$ of $R^Z_{C_1,C_2}$, $\omega^\kappa D_{\overline{a},\overline{a}}\in S^\perp$ exactly when $\overline{a}\in C_2^\perp$ as from Theorem \ref{stable} for any $c\in C_2$ $D_{\overline{0},c}\in S$ and hence
% \begin{equation*}
% 0=(\overline{a},\overline{a})\star(\overline{0},c)=\lan\overline{a},c\ran
% \end{equation*}
% hend $\overline{a}\in C_2^\perp$.
\end{proof}

The next result follows identically.

\begin{thm}\label{error phase}
Let $C_2\subset C_1\subset\mathbb{F}_d^n$ be linear subspaces, then the codes $R^X_{C_1,C_2}$ and $R^Z_{C_1,C_2}$ can correct up to $t$ single-qudit flip, phase and phase-flip errors where
\begin{equation*}
t=\op{min}\left\{\left\lfloor\frac{\op{wt}(C_1)-1}{2}\right\rfloor,\left\lfloor\frac{\op{wt}(C^\perp_2\setminus C_1)-1}{2}\right\rfloor\right\}.
\end{equation*}
\end{thm}

For some simple examples of this theorem in action the reader is referred back to Example~\ref{shors} and Example~\ref{3perfect}. The following remark and example gives the best possible encoding rate for an extended reflexive code. 

\begin{rem}\label{minimals}
The basic principal in quantum error correction is the concept that each error transforms distinct code words into distinct orthogonal subspaces. This becomes quite restrictive on the minimal length in which one can embed into. This is the topic of a later paper. For now, we present this minimal length for a specific example, namely the case of a 4-state system (see Example~\ref{4statex}). To protect from any flip or phase error on a 4-state system, the space requires an orthogonal subspace for each of the 6, 3 flips and 3 phases, errors plus one for the unperturbed state. This makes a total of $6n+1$. We must quadruple this to have enough space to accommodate for each of the 4 embedded states; i.e. $k=1$ logical qudits. Thus, the number of subspaces is $4(6n+1)$. To have enough room in the Hilbert space we have the condition:
\begin{equation*}
4(6n+1)\leq 4^n
\end{equation*}
for which the smallest number satisfying this equation is $n=4$. The next example gives a reflexive stabilizer code which meets this lower bound.
\end{rem}
\begin{ex}\label{4statex}
We will consider codes in field with four elements, which we denote as
\begin{equation*}
\mathbb{F}_4=\{0,1,x,x+1\}
\end{equation*}
where $x^2+x+1=0$. Let $C_1\subset\mathbb{F}_4^4$ be the 2-dimensional code consisting of the following vectors:
\begin{center}
\begin{tabular}{cccccccc}
$0000$,&$1x10$,&$xx^2x0$,&$x^21x^20$,&$x^2x^201$,&$110x$,&$xx0x^2$,&$x111$\\
$x^2xxx$,&$1x^2x^2x^2$,&$10x1$,&$x0x^2x$,&$x^201x^2$,&$0x^21x$,&$01xx^2$,&$0xx^21$.
\end{tabular}
\end{center}
We then set $C_2=\{0000,x111,x^2xxx,1x^2x^2x^2\}$ and hence our code words for the flip-error extended RSC $R_{C_1,C_2}^X$ are given by 
\begin{equation*}
\begin{split}
|\Psi_{0000}\ran+|\Psi_{x111}\ran+|\Psi_{x^2xxx}\ran+|\Psi_{1x^2x^2x^2}\ran\\
|\Psi_{1x10}\ran+|\Psi_{x^2x^201}\ran+|\Psi_{x0x^2x}\ran+|\Psi_{01xx^2}\ran\\
|\Psi_{10x1}\ran+|\Psi_{x^21x^20}\ran+|\Psi_{xx0x^2}\ran+|\Psi_{0x^21x}\ran\\
|\Psi_{xx^2x0}\ran+|\Psi_{0xx^21}\ran+|\Psi_{110x}\ran+|\Psi_{x^201x^2}\ran
\end{split}
\end{equation*}
By Theorem \ref{error ext}, one easily checks that this code can correct any single-qudit flip or phase error which, by Remark \ref{minimals}, is the minimal such code for a 4-state system.
\end{ex}


==> eccs.tex <==
\section{Quantum Error Correcting Codes} 

\subsection{Error correction on the $n$-tensor / Introduction to Error Correcting Codes and/or Stabilizer Codes}


\subsection{Error correction on Fock Space}
\RV{put stuff about del x and del x star}

==> ext.tex <==
\subsection{Extension of reflexive codes}\label{ext}
In Section \ref{error correction} we see that reflexive codes, have limitations in error correction, to overcome these limitations we extend these reflexive codes. This extension is a similar to CSS codes \cite{goodcodes,ortho}. We establish two extensions that protect against phase and flip errors, respectively. 

\begin{defn}\label{just ok}
Let $C_2\subset C_1\subset\mathbb{F}_d^n$, be linear subspaces and let $R_{C_1}=\{|\Psi_c\ran \}$ be the Reflexive QECC associated to $C_1$. We then define two extensions of reflexive codes. The first will be referred to as a \textbf{phase-error extension by $\mathbf{C_2}$}, and is the quantum code generated by
\begin{equation*}
R^Z_{C_1, C_2}:=\left.\left\{|\Phi_{c'}\ran:=\frac{1}{\sqrt{|C_2|}}\left(\sum_{c\in C_2}D_{\overline{0},c}|\Psi_{c'}\ran\right)\,\right|\,c'\in C_1\right\}.
\end{equation*}
The second extension will be referred to as an \textbf{flip-error extension by $\mathbf{C_2}$}, and is the quantum code generated by
\begin{equation*}
R^X_{C_1, C_2}:=\left.\left\{|\Phi_{c'}\ran:=\frac{1}{\sqrt{|C_2|}}\left(\sum_{c\in C_2}D_{c,\overline{0}}|\Psi_{c'}\ran\right)\,\right|\,c'\in C_1\right\}.
\end{equation*}
One sees that in either case, two of the above code words $|\Phi_c\ran$ and $|\Phi_{c'}\ran$ match if and only if $c-c'\in C_2$, and hence the dimension of $R^X_{C_1,C_2}$ (or $R^Z_{C_1,C_2}$) is $\op{dim}_{\mathbb{F}_d}(C_1)-\op{dim}_{\mathbb{F}_d}(C_2)$.
\end{defn}

\begin{thm}\label{stable}
Let $C_2\subset C_1\subset\mathbb{F}_d^n$ be a linear subspaces, then both $R^X_{C_1,C_2}$ and $R^Z_{C_1,C_2}$ are stabilizer codes, and the stabilizer is generated by the elements of $S_{C_1^\perp}$ and $\left.\Big\{D_{\overline{0},c}\,\right|\,c\in C_2\Big\}$ for $R^Z_{C_1,C_2}$, and  $S_{C_1^\perp}$ and $\left.\Big\{D_{c,\overline{0}}\,\right|\,c\in C_2\Big\}$ for $R^X_{C_1,C_2}$.
\end{thm}
\begin{proof}
We will only show the result for $R^Z_{C_1,C_2}$ as the other follows similiarly. First, note that for any $\overline{a}\in C_1^\perp$ and $c\in C_2$, the operators  $D_{\overline{a},\overline{a}}\in S_{C_1^\perp}$ and $D_{\overline{0},c}$ commute because 
\begin{equation*}
(\overline{a},\overline{a})\star(\overline{0},c)=\lan\overline{a},c\ran=0
\end{equation*}
since $a\in C_1^\perp$. Now we show that for any $c\in C_2$ and $c'\in C_1$ that $D_{\overline{0},c}|\Phi_{c'}\ran=|\Phi_{c'}\ran$. This follows from the observation that for $m=1$ for any $\alpha,\beta\in\mathbb{F}_p$ that $Z(\alpha)|\psi_\beta\ran=|\psi_{\beta-\alpha}\ran$ so 
\begin{equation*}
D_{\overline{0},c}|\Psi_{c'}\ran=|\Psi_{c'-c}\ran.
\end{equation*}
The result for general $m$ is follows and thus the result follows.
\end{proof}
The next results is an immediate consequence.
\begin{cor}\label{stables}
Let $C_2\subset C_1\subset\mathbb{F}^n_d$ be linear subspaces, and $S_X$ be the stabilizer for $R^X_{C_1,C_2}$ and $S_Z$ be the stabilizer for $R^Z_{C_1,C_2}$ then we have
\begin{equation*}
S_X^\perp:=\left.\Big\{\omega^k D_{a,b}\,\right|\;a-b\in C_1\,\text{ and }\,a\in C_2^\perp\Big\}
\end{equation*}
\begin{equation*}
S_Z^\perp:=\left.\Big\{\omega^k D_{a,b}\,\right|\;a-b\in C_1\,\text{ and }\,b\in C_2^\perp\Big\}
\end{equation*}
where $S^\perp$ is the set of operators which commute with operators in $S$.

\end{cor}
\begin{rem}\label{just css}
One will notice that CSS codes are in one-to-one correspondence with extended reflexive codes via another choice of error basis. That is, an error basis which was instead generated by $Y$ and $Z$ from Example \ref{qubit basis}, and obtained if we were to define:
\begin{equation*}
\tilde{D}_{\overline{a},\overline{b}}=\bigotimes_{i=1}^n Y^{a_i}Z^{b_i}.
\end{equation*}
That is to say sticking with the standard basis on $\mathbb{F}_2^{2n}$, the parameter space of the Error Basis, we can build a linear isomorphism
\begin{equation*}
\begin{split}
\mathbb{F}_2^{2n}&\mapsto\mathbb{F}_2^{2n}\\
(a,a)&\mapsto (a,0)\\
(b,0)&\mapsto (0,b).
\end{split}
\end{equation*}
It is now a simple exercise to show that the above isomorphism takes the stabilizer for a reflexive stabilizer code $R^X_{C_1,C_2}$ (with $d=2$) to a stabilizer of a CSS code. In the following section we show that reflexive stabilizer codes have the same correction capabilities for single-qubit errors.
\end{rem}

The next two examples help elucidate the application Definition~\ref{just ok}. Moreover, these examples utilize well-known classical and quantum codes, providing context for reflexive codes. 

\begin{ex}\label{shors}
Our next example uses the classical example of the [7,4,3]-Hamming code, that is the linear subspace of $\mathbb{F}_2^7$ consisting of the following vectors:
\begin{equation}\label{hammingcode}
\begin{split}
0000000,0001011,0010110,0011101,\\
0100111,0101100,0110001,0111010,\\
1000101,1001110,1010011,1011000,\\
1100010,1101001,1110100,1111111.
\end{split}
\end{equation}
Shor used this code in \cite{goodcodes} to build a quantum stabilizer code which encoded one qubit into seven qubits.

For reflexive codes, we will embed three qubits into the seven qubits. We set $C_1$ as the classical Hamming code given in Equation~\eqref{hammingcode} and we set $C_2=\op{span}_{\mathbb{F}_2}(1111111)$. Then $C_2^\perp$ consists of all elements of $\mathbb{F}_2$ with even Hamming weight. It follows from Theorem \ref{error ext} that our code will correct any single-qubit flip or phase error. From Definition~\ref{just ok}, we find the code words for the flip-error extended code $R_{C_1,C_2}^X$
\begin{equation*}
\begin{split}
|\Psi_{0000000}\ran+|\Psi_{1111111}\ran,&\;\;|\Psi_{0001011}\ran+|\Psi_{1110100}\ran,\\
|\Psi_{0010110}\ran+|\Psi_{1101001}\ran,&\;\;|\Psi_{0011101}\ran+|\Psi_{1100010}\ran,\\
|\Psi_{0100111}\ran+|\Psi_{1011000}\ran,&\;\;|\Psi_{0101100}\ran+|\Psi_{1010011}\ran,\\
|\Psi_{0110001}\ran+|\Psi_{1001110}\ran,&\;\;|\Psi_{0111010}\ran+|\Psi_{1000101}\ran.
\end{split}
\end{equation*}

One could write out these code words using the computational basis, as in Example~\ref{something}, but doing so would be cumbersome as each is a linear combination of 58 basis elements.
This example encodes three times the information as Shor's code given in \cite{goodcodes} but cannot correct phase-flip errors by Theorem~\ref{error phase}. 
\end{ex}

\begin{ex}\label{3perfect}
Now, we provide an extended RCS which obtains the same rate as the [5,1,3]-Perfect Code introduced in \cite{perfect}. Unlike the Perfect Code, the code presented here is on a 3-state system. Let $C_1\subset\mathbb{F}_3^5$, be the 2-dimensional code consisting of the following vectors:
\begin{equation*}
00000,11111,22222,00211,00122,11200,11022,22100,22011
\end{equation*}
Similar to Example \ref{shors} above, we choose $C_2=\op{span}_{\mathbb{F}_3}(11111)$. Hence the extended flip-error extended code $R_{C_1,C_2}^X$ has code words:
\begin{equation*}
\begin{split}
|\Psi_{00000}\ran+|\Psi_{11111}\ran+|\Psi_{22222}\ran,\\
|\Psi_{00211}\ran+|\Psi_{11022}\ran+|\Psi_{22100}\ran,\\
|\Psi_{00122}\ran+|\Psi_{11200}\ran+|\Psi_{22011}\ran.
\end{split}
\end{equation*}
By Theorem \ref{error ext}, one easily checks that this code can correct any single-qudit flip or phase error. Thus this code embeds one logical qudit into five physical qubits and corrects any single-qudit flip or phase error. Notice that cannot correct against single-qudit flip-phase errors, by Theorem \ref{error phase}, and therefore does not match the correction capability of the Perfect Code \cite{perfect}. 
\end{ex}


\begin{defn}\label{good}
Let $C\subset\mathbb{F}_d^n$, and $c\in C$ be a non-zero element, such that for each $i\in\{1,\ldots,n\}$ where $c_i=0$ for each $c'\in C\setminus\{ac\,|\,a\in\mathbb{F}^*_d\}$ we can find $\epsilon_{c'}\in\{0,\ldots,p-1\}$ so that $\omega^{\kappa_{c'_i}+\epsilon_{c'}}=\omega^{\kappa_{c''_i}+\epsilon_{c''}}$ for every $c',c''\in C\setminus\{ac\,|\,a\in\mathbb{F}^*_d\}$ we then define the quantum code generated by
\begin{equation*}
R^c_C=\left.\left\{|\varphi_{c'}\ran:=\frac{\omega^{\epsilon_{c'}}}{\sqrt{d}}\left(\sum_{a\in\mathbb{F}_d}|\Psi_{c'+ac}\ran\right)\,\right|\,c'\in C\setminus\{ac\,|\,a\in\mathbb{F}^*_d\}\right\}
\end{equation*}
Again, one sees that two of the above code words $|\varphi_{c''}\ran$ and $|\varphi_{c'}\ran$ match if and only if $c'-c''\in \{ac\,|a\in\mathbb{F}_d\}$, and hence the dimension of $R^{c}_{C}$ is $\op{dim}_{\mathbb{F}_d}(C_1)-1$.
\end{defn}
\begin{rem}
At first glance one may worry that these codes would be too much trouble to find yet anytime there exists a $c\in C$ such that $w(c)=n$ the conditions are trivially met. As well in practice when $w(c)=n-1$ it is not too much work to make the above conditions hold. As well, besides the coefficients the codes from Definition \ref{good} and Definition \ref{just ok} look identical, but these coefficients will be leveraged in the next section to guarantee larger error correction capabilities.
\end{rem}

==> gates.tex <==
\section{Fault Tolerant gates}
blah.. define the set $\mathcal{C}:=\left\{ \right\}$...Now, using the ideas from \cite{fault,ortho,shorfault} we make the following definition. 

\RV{obviously this section is for fault tolerant gates}

\RV{OR WE CAN LEAVE THESE LAST TWO SECTIONS AS THEIR OWN PAPER(S) AND JUST END WITH A QUANTUM GV-BOUND??? WHICH COULD ANSWER A QUESTION FROM SHOR'S PAPER \cite{ortho}}

==> gv.tex <==
\section{GV-Bound}

\RV{ QUANTUM GV-BOUND??? WHICH COULD ANSWER A QUESTION FROM SHOR'S PAPER \cite{ortho}}

\RV{I say we don't even bother for this first paper... lets just get these codes out there!!}

==> newschema.tex <==
\RV{again I changed this name from compression}
\section{Error correction for quantum communication}
Next we will develop our error correction protocol on indeterminate-length codes. The main inspiration for this protocol comes from \cite{real} where they present different realizations of indeterminate-length codes into physical spaces. We will use just one of these realizations that work best for our protocol, which we present next.

\subsection{Realizing indeterminate-length messages}
From Section \ref{old error} we see that error correction (for stabilizer codes) were developed for block codes, i.e. codes with a fixed qubit length. Thus to use this existing technique we will first have to realize our indeterminate-length codes in a physical space $\mathcal{H}$. First set an indeterminate-length code $W:H\ra T(\C^d)$, where $H$ is the source, and denote $\lmax=\lmax(W)$. Assuming $\mathcal{H}$ is a system of $k$-qudits, for some $k\in\N$, thus $d^k=\dim \mathcal{H}$, one  must have
\begin{equation*}
\dim(\mathcal{H})\geq \dim\left(T^{\leq \lmax}(\C^2d)\right)
\end{equation*}
\begin{equation*}
\implies \sum_{i=0}^{\lmax} d^i=\frac{d^{\lmax+1}}{d-1}\leq d^k
\end{equation*}
\begin{equation*}
\implies k\geq\lmax+1.
\end{equation*}
Inspired from classical computers and the work of \cite{real}, we now define a length $\ell$ realization morphism and its partial inverse.
\begin{defn}
For $\ell\in\N$, we denote the $\ell^{\text{th}}$-realization morphism (or $\ell^{\text{th}}$-realization for the sake of brevity)
\begin{equation*}
\mathcal{R}_\ell:T^{\leq \ell}(\C^d)\ra\left(\C^d\right)^{\otimes \ell+1}
\end{equation*}
defined for a length eigenstate $|\psi\ran\in T^{\leq \ell}(\C^d)$, with $\op{len}(|\psi\ran)=m\leq\ell$ as \RV{make sure to define $\op{len}$ earlier!}
\begin{equation*}
\mathcal{R}_{\ell}(|\psi\ran):=| \underbrace{0\,...\,0}_{\ell-m}1\psi\ran,
\end{equation*}
and extend $\mathcal{R}_\ell$ by linearity. That is, we adjoin the prefix  1 to indicate the beginning of the code word and adjoining an additional $\ell-m$ number of 0's to ensure that $\mathcal{R}_\ell(|\psi\ran)\in\left(\C^2\right)^{\otimes \ell+1}$. This morphism clearly has a partial inverse which we will denote 
\begin{equation*}
\mathcal{R}\inv_{\ell}:\left(\C^2\right)^{\otimes \ell+1}\ra T^{\leq\ell}(\C^2)\subset T\left(\C^2\right).
\end{equation*}

\end{defn}
\begin{ex}
blah...
\end{ex}


==> noise.tex <==
\section{Noisy Shannon (perhaps just say channel) bounds}

\RV{The idea for this section is to walk the reader through, how if they have a multivariate distribution approximated for the errors of their channels how to build a reflexive code that will give them the optimal correction for their noisy channel}

==> qcomp.tex <==
\section{Quantum Information Theory}

\RV{Section may need new name.. used to be called quantum compression}
%First, we denote the so called, \emph{computational basis}, as is standard, by $|0\ran:=\begin{bmatrix}1\\ 0 \end{bmatrix}$ and $|1\ran:=\begin{bmatrix}0\\1 \end{bmatrix}$.  Therefore any quantum state of a single qubit system may be expressed as $|\psi\ran=\alpha|0\ran+\beta|1\ran\in\C^2$, for some $\alpha,\beta\in\C$ such that $|\alpha|^2+|\beta|^2=1$ (i.e. the \emph{Born rule}). 


\RV{I started the long process of making this $d$-ary instead of binary!}
In what follows, all codings will be done into strings of dits or strings of qudits for classical and quantum codes, respectively. Therefore all codewords will be strings of elements from a $d$-ary alphabet $A$ such that $|A|=d\in\N$ (in the classical case) or, possibly the superposition of, strings from a quantum $d$-ary alphabet $\mc A$ which is an orthonormal basis of the Hilbert space $H_{\mc A}=\C^d$ (in the quantum case). Everything that follows is easily applied to the case of $d$-ary alphabets, that is dits and qudits.

\subsection{Classical Codes and the Kraft Inequality}

Let $S$ be a finite or countable set equipped with the power set $\sigma$-algebra $\mc P(S)$, and let $X$ be a random variable with values in $S$. 
The set $S$ will be referred to as the \textbf{symbol set} that we wish to encode. 
In the literature, the set $S$ is referred to as the set of objects, the message set, or sometimes even the index set. 
For any set $Y$, we will set $Y^+$ equal to the set $\cup_{\ell=0}^\infty Y^{\ell}$ which is the collection of all possible finite strings from $Y$, where $Y^0$ denotes the empty set (or empty string). 
%Lastly, let $A=\{0,1\}$ be the $d$-ary alphabet. Already named A above
A \textbf{code} $C:S\ra A^+$ is a mapping from $S$ to $A^+$, the set of finite strings with letters in the $d$-ary alphabet $A$. 
The range of the code, $A^+$, is referred to as the \textbf{codebook} and its elements are the \textbf{codewords}. 
Moreover, for each $x\in S$, we refer to $C(x)$ as the \textbf{codeword of the symbol \bma{$x$}}. 
For each $a\in A^+$, we call the \textbf{length of \bma{$a$}} (denoted by $\ell(a)$) the unique integer $m$ such that $a\in A^m$. 
%We define $\ell: A^+\ra \N_0$, where $\N_0=\N\cup \{0\}$, as the unique integer $m$ whenever $a\in A^m$ and refer to $\ell(a)$ as the . 
%For notational convenience, we will set $\ell(x)=\ell(C(x))$ for any $x$ in a set of symbols $S$ with a source code $C$ and refer to $\ell(x)$ as the \textbf{length} of $x$. 
%Furthermore, we will often enumerate the elements of $S=\{x_1,x_2,\ldots, x_m\}$ and denote the length of $x_i$ by $\ell_i$. 

The \textbf{expected length} of a code $C$ on a symbol set $S$ is given by 
\begin{equation*}\label{expected length}
EL(C):= \sum_{x\in S}p(x)\ell(C(x))=\E[\ell (C (X))],
\end{equation*}

\noindent where $p:S\ra [0,1]$ is the probability mass function (pmf) of the random variable $X$ and the expectation $\E$ is taken with respect to $p$. 
%Furthermore, it is common in the literature to refer to the pmf $p$ of $X$ as the \textbf{source code distribution} and we adopt that convention throughout. 

%In lossless coding, we are only interested in injective codes; $C$ is injective whenever 
%\begin{equation*}\label{non-singular}
%x\ne y \Ra C(x)\ne C(y),\quad \text{for all }x,y\in S;
%\end{equation*}
%
%\noindent and hence the codewords are pairwise distinguishable. 
We extend the code $C$ by concatenation to obtain the \textbf{extended code}, also called the extension of $C$, $C^+: S^+\ra A^+$. That is to say 
\begin{equation*}\label{extended code}
C^+(x_1x_2\cdots x_n)=C(x_1)C(x_2)\cdots C(x_n)\quad \text{for all }x_1x_2\cdots x_n\in S^n\text{ and } n\in\N, 
\end{equation*}

\noindent and we define $C^+(\emptyset)=\emptyset$. 
We call the code $C$ \textbf{uniquely decodable} whenever its extension $C^+$ is injective; i.e.\ $C$ is uniquely decodable whenever all strings of symbols from $S$ are pairwise distinguishable. 
In lossless coding we are only interested in uniquely decodable codes. 

An extremely useful class of uniquely decodable codes are the so-called \textbf{instantaneous (or prefix-free)} codes. A code is said to be prefix-free if no codeword is the prefix of another; i.e.\ for every distinct pair $x,y\in S$ there is no $a\in A^+$ such that $C(x)a=C(y)$. Prefix-free codes are called instantaneous because the decoder is able to read out each codeword from a string of codewords, instantaneously, as soon as she sees that word appear in a string (without waiting for the entire string). 


\DW{The remainder of this subsection is probably unnecessary unless we are able to introduce some type of optimality.} 
The Kraft-McMillan Inequality is fundamental in classical data compression.
\RV{this was wrong the way it was stated... I've corrected it and updated using $d$ for alphabet size}
\begin{thm}(Kraft-McMillan Inequality, \text{\cite[Theorems 5.2.1 and 5.5.1]{CT91}})\label{Kraft}
	For any uniquely decodable code over an alphabet $A$ with cardinality $|A|=d\in \N$, with codeword lengths $\ell_1,\ell_2,\ldots, \ell_n$ must satisfy the inequality $$\sum_{i=1}^n d^{-\ell_i}\le 1.$$
	Conversely, given a set of codeword lengths that satisfies this inequality, there exists an instantaneous code with these code lengths. 
\end{thm}

\RV{SERIOUSLY???!!! am I missing something isn't this obvious? why in the world would you need any of these assumptions or even waste paper writing the conversely??}

\begin{Rem}
	The Kraft-McMillan Inequality is sometimes referred to only as the Kraft Inequality. 
	%However, the inequality as stated above (for uniquely decodable codes) was first proved by B. McMillan in 1956 in \cite{Mcmillan56}. 
	This is due to the fact that Kraft was the first to prove the inequality in \cite{Kraft49}, although his original result refers only to instantaneous codes. McMillan later extended Kraft's work to include all uniquely decodable codes in \cite{Mcmillan56}. 
	Furthermore, it is worth noting that the Kraft-McMillan inequality can be extended to a countable set of symbols (see Theorem~5.2.2 and the corollary following Theorem~5.5.1 in \cite{CT91}). When including countable sets of symbols, the inequality is referred to as the Extended Kraft-McMillan Inequality. 
\end{Rem}

An immediate corollary to the Kraft-McMillan Inequality is the following:

\begin{Cor}
	Given any uniquely decodable code with codeword lengths $\ell_1,\ell_2,\ldots, \ell_m$, there exists an instantaneous code with these same code lengths. 
\end{Cor}

We call a uniquely decodable code $C$ \textbf{optimal} whenever the expected length $EL(C)$ is minimized; i.e.\ the optimal uniquely decodable code is given by 
\begin{equation}\label{optimality}
\begin{split}
C_{\text{opt}}:&= \argmin_C \{EL(C) : C\text{ is uniquely decodable}\} \\
&= \argmin_C \{EL(C) : \text{the codeword lengths of the }C\text{ satisfy} \sum_i 2^{-\ell_i}\le 1\},
\end{split}
\end{equation}
where the last equality follows from Theorem~\ref{Kraft}. 
We set $EL^*(X):=EL(C_{\text{opt}})$ the \textbf{optimal expected length of the random variable \bma{$X$}}. 
The results for the optimal expected length are summarized in the following: 

\begin{Thm}(\text{\cite[Theorem 5.4.1]{CT91}})\label{optimal code}
	Let $X$ be a random variable with range in the symbol set $S$. 
	Then the optimal expected length of $X$ satisfies the inequality 
	$$H(X)\le EL^*(X)<H(X)+1,$$ 
	where $H(X)$ is the Shannon entropy of $X$, i.e.\ $H(X)=-\sum_{i\in S} p_i\log_2 p_i$ where $(p_i)_{i\in S}$ is the pmf of $X$. 
\end{Thm}

\noindent Well known examples of codes which satisfy the inequality of Theorem~\ref{optimal code} are the so-called Huffman codes and Shannon-Fano codes. 

In the above theorem, we are only interested in the compressability of single codewords. Suppose instead that we wish to compress strings of codewords with code distributions given by a stochastic process $\X=(X_i)_{i=1}^\infty$. 
Then, for each $n\in \N$, Theorem~\ref{optimal code} holds for the random vector $(X_1,X_2,\ldots, X_n)$, giving 
$$ H(X_1,X_2,\ldots, X_n)\le EL^*(X_1,X_2,\ldots,X_n)< H(X_1,X_2,\ldots, X_n)+1.$$ 
For each $n\in\N$, we set 
\begin{equation}\label{expected length n}
EL^*_n(\X):=\frac{1}{n}EL^*(X_1,X_2,\ldots, X_n)
\end{equation} 
to be the \textbf{optimal expected codeword length per symbol} for the first $n$ symbols. 
We can then express the optimal expected codeword length per symbol (over all symbols) in terms of the entropy rate, which is a dynamical entropy for stochastic processes. The \textbf{entropy rate} of a stochastic process $\X=(X_n)_{n=1}^\infty$ is given by 
\begin{equation*}
H(\X)=\lim_{n\ra\infty} \frac{1}{n} H(X_1,\ldots, X_n), 
\end{equation*} 
whenever the limit exists. There are many instances when it is known that the above limit exists (e.g.\ stationary stochastic processes, see \cite[Theorem 4.2.1]{CT91}). %\cite[Page 60]{CT91} for definition). 

\begin{Thm}(\text{\cite[Theorem 5.4.2]{CT91}})\label{expected per symbol}
	The optimal expected codeword length per symbol for a stochastic process $\X=(X_i)_{i=1}^\infty$ satisfies 
	\begin{equation*}
	\frac{H(X_1,X_2,\ldots, X_n)}{n}\le EL^*_n(\X) < \frac{H(X_1,X_2,\ldots, X_n)}{n}+\frac{1}{n}.
	\end{equation*}
	Moreover, if $\X$ is such that the limit defining entropy rate exists (e.g.\ $\X$ is a stationary stochastic process), then 
	\begin{equation*}
	EL_n^*(\X)\ra H(\X)\quad\text{as }n\ra\infty.
	\end{equation*}
	%where $H(\X)$ is the entropy rate of the stochastic process $\X$. 
	In particular, if $\X$ consists of independent identically distributed (i.i.d.) copies of a random variable $X$, then 
	\begin{equation*}
	EL_n^*(\X)\ra H(X)\quad\text{as }n\ra\infty.
	\end{equation*} 
\end{Thm}

This finishes our brief overview of data compression in classical information theory. For a more detailed exposition see \cite[Chapter 5]{CT91}. 
%{\color{red} Depending on what all we include in this paper, we may need to add things such as \cite[Theorem 5.4.3]{CT91}.} 



\RV{I think this needed a new title as well previously called Quantum Data compression}
\subsection{Quantum Communication}\label{Q Data Compression}


We begin with the description of indeterminate-length quantum codes, whose preliminary investigation began with Schumacher \cite{Schumacher94} and Braunstein et.\ al in \cite{BFGH00}, and they were formalized in \cite{SW01}. 
%We may think of the codes introduced in the previous section as being varying-length codes; 
The term indeterminate-length is used to draw attention to the fact that a quantum code must allow for superpositions of codewords, including those superpositions containing codewords with different lengths. 
We will follow the formalisms in \cite{AW19} (which is similar to that of \cite{BBHZ17} and \cite{MR08}) as opposed to the zero-extended forms of \cite{SW01}. 
A description of the connection between these two formalisms can be found in \cite{BF02}. 

For any Hilbert space $H$, we will denote by $T(H):=\oplus_{\ell=0}^\infty H^{\ten \ell}$ the \textbf{free Fock space or tensor algebra} over $H$, where $H^{\ten 0}=\C$. 
We will denote the scalar $1\in H^{\ten 0}$ by $|\emptyset\rangle$ and refer to it as the \textbf{empty string}. 
\DW{I'm not sure whether or not we will include ensembles of general type in our paper. Up to now we have only considered ensembles which are made up of orthogonal codewords.} 
Let $\mc S=\{p_n,|s_n\rangle\}_{n=1}^N$ be an \textbf{ensemble of pure states}, or simply ensemble, where $p=\{p_n\}_{n=1}^N$ is the pmf of a random variable $X$ and $|s_n\rangle$ is an element of a $d$-dimensional Hilbert space $H_\mc S$, for each $1\le n\le N$, such that $H_{\mc S}=\span\{|s_n\rangle\}_{n=1}^N$. 
The collection $\{|s_n\rangle\}_{n=1}^N$ will be referred to as the \textbf{symbol states} of the ensemble $\mc S$. 
An \textbf{(indeterminate-length) quantum code}, $U$, over a quantum $d$-ary alphabet $\mc A$, which is an orthonormal basis for $H_\mc A=\C^d$, is a linear isometry $U:H_\mc S\ra T(H_{\mc A})$. 
\DW{I like this convention, but it probably needs to be introduced in a smoother manner. 
In the sequel, we will set $T:= T(H_{\mc A})=T(\C^2)=\C\langle x,y\rangle$ where $\C\langle x,y\rangle$ is the collection of polynomials over $\C$ with non-commuting variables $x$ and $y$. Indeed, we may not even need to introduce extended codes or $T(H)$ for a general Hilbert space $H$ depending on our results.} 
The \textbf{extended quantum code of \bma{$U$}} is the linear mapping $U^+:T(H_\mc S)\ra T$ given by 
\begin{equation*}
	U^+(|s_1 s_2\cdots s_n\rangle)=U(|s_1\rangle)U(|s_2\rangle)\cdots U(|s_n\rangle),
\end{equation*}

\noindent for all $|s_1 s_2\cdots s_n\rangle \in H_\mc S^{\ten n}$ and $n\in\N$, and we set $U^+(|\emptyset\rangle)=|\emptyset\rangle$, where concatenation is defined according to \cite[Definition 2.3]{MR08} (see also \cite[Section V]{MRN09}). 

The quantum code $U$ is said to be \textbf{uniquely decodable} if the extended quantum code $U^+$ is an isometry. 
Throughout this paper, we will restrict ourselves only to the situation where the range \DW{(or image as Rob likes to refer to it)} of $U$ is a subset of $\oplus_{\ell=0}^{\lmax} H_{\mc A}^{\ten \ell}$ for some $\lmax\in \N$; i.e.\ there is a finite upper bound $\lmax$ on the length of all codewords. 



\begin{rem}
	The authors of \cite{BF02} allow non-empty strings to map to the empty string. In their paper, the authors send along a classical side channel to give the lengths of the codewords and so that convention is possible. Without the classical side channel (as is the approach in the present paper) allowing non-empty strings to map to the empty string will cause the quantum code to \textit{not} be uniquely decodable.
\end{rem}

Let $\mc S=\{p_n,|s_n\rangle\}_{n=1}^N$ be an ensemble whose symbol states $\{|s_n\rangle\}_{n=1}^N$ span a Hilbert space $H_{\mc S}$ of dimension $k$. 
Consider a classical uniquely decodable code, $C$, on a symbol set, $S=\{x_i\}_{i=1}^k$, with $k$-many symbols. 
We will construct a corresponding uniquely decodable quantum code, $U$, from $C$ by identifying the classical $d$-ary alphabet $A$ with the quantum $d$-ary alphabet $\mc A\subseteq \C^d$ and the symbol set, $S$, with any orthonormal basis $\{|e_i\rangle\}_{i=1}^k$ of $H_\mc S$; this construction is given in \cite{BBHZ17} and \cite{AW19}. 
Fix an orthonormal basis $\{|e_i\rangle\}_{i=1}^k$ of $H_\mc S$ and define the quantum code $U:H_\mc S\ra H_{\mc A}^\oplus$ by the equation
\begin{equation}\label{C-Q source code}
	U=\sum_{i=1}^d |C(x_i)\rangle\langle e_i|.
\end{equation}
It is clear that $|C(x_i)\rangle \in H_\mc A^{\ten \ell_i}\subseteq H_\mc A^\oplus$, where $\ell_i$ is the length of $C(x_i)$, and that $\{|C(x_i)\rangle\}_{i=1}^k$ is an orthonormal set, so that $U$ is a linear isometry. Furthermore, since $C$ is uniquely decodable, the map $U^\ell:H_\mc S^{\ten\ell}\ra H_\mc A^\oplus$ defined by the equation 
\begin{equation*}\label{C-Q ext source code1}
	U^\ell =\sum_{i_1=1}^d\cdots \sum_{i_\ell=1}^d |C(x_{i_1})C(x_{i_2})\cdots C(x_{i_\ell})\rangle\langle e_{i_1}e_{i_2}\cdots e_{i_\ell}|
\end{equation*}
is a linear isometry for each $\ell\in\N$. 
Since the extended quantum code $U^+:H_\mc S^\oplus\ra H_\mc A^\oplus$ is given by 
\begin{equation*}\label{C-Q ext source code2}
	U^+=\sum_{\ell=0}^\infty U^\ell, 
\end{equation*}
we see that $U^+$ is a linear isometry and hence $U$ is uniquely decodable. We will refer to quantum codes constructed from classical ones by Equation~\eqref{C-Q source code} as \textbf{classical-quantum encoding schemes (c-q schemes)}. 
(In \cite{BBHZ17} c-q schemes are referred to as \textit{lossless quantum encoding schemes}.)

\DW{Again, as of yet we have only discussed those symbol states which are indeed orthogonal.} 
\begin{rem}
	Notice that the symbol states $\{|s_n\rangle\}_{n=1}^N$ of the ensemble $\mc S$ are not directly encoded by the $|C(x_i)\rangle$'s unless $N=d$ and there exists a permutation $\sigma$ of $\{1,\ldots, d\}$ such that  $|s_{\sigma(i)}\rangle=|e_i\rangle$ for every $i\in\{1,\ldots, d\}$. In fact $U|s_n\rangle$ need not belong to $H_\mc S^{\ten\ell}$ for any $\ell\in\N$, but can in general be in a superposition of different lengths. (Hence the term indeterminate-length quantum codes.)
\end{rem} 


\DW{Quantum Kraft-McMillan Inequality and remainder of section probably need not be mentioned unless we have optimality results.} 
The Kraft-McMillan Inequality (Theorem~\ref{Kraft}) was initially extended to the quantum domain in \cite{SW01} and subsequently in \cite{MR08} and \cite{BBHZ17}. Before presenting (a slightly different) Quantum Kraft-McMillan Inequality, we will first introduce the length observable and quantum codes with length eigenstates. The \textbf{length observable} $\Lambda$ acting on $H_\mc A^\oplus$ is given by 
\begin{equation}\label{length observable}
	\Lambda:= \sum_{\ell=0}^\infty \ell \Pi_\ell,
\end{equation}
where $\Pi_{\ell}$ is the orthogonal projection onto the subspace $H_\mc A^{\ten\ell}$ of $H_\mc A^\oplus$. 

We say that a quantum code $U: H_\mc S\ra H_{\mc A}^\oplus$ has \textbf{length eigenstates} if $U$ has the form 
\begin{equation}\label{length eigenstates}
	U=\sum_{i=1}^d |\psi_i\rangle\langle e_i|.
\end{equation}
for some orthonormal basis $\{|e_i\rangle\}_{i=1}^d$ of $H_\mc S$ and some sequence $\{|\psi_i\rangle\}_{i=1}^d\subseteq H_{\mc A}^+$ such that, for each $1\le i\le d$, $|\psi_i\rangle\in H_{\mc A}^{\ten \ell_i}$ for some $\ell_i\in\N$. 

Note that the $|\psi_i\rangle$'s are orthogonal due to $U$ being a linear isometry. It is easy to see that every c-q scheme is a quantum code with length eigenstates. 
Lastly, for each $\ell\in\N\cup\{0\}$, we will refer to the elements of the set $\{\psi_i: i\in\{1,\ldots,d\},\ \psi_i\in H_{\mc A}^{\ten \ell}\}$ as the \textbf{length \bma{$\ell$} eigenstates of \bma{$U$}} and we will refer to $\{\ell_i\}_{i=1}^d$, where, for each $i=1,\ldots, d$, $\psi_i\in H_{\mc A}^{\ten \ell_i}$, as the \textbf{length eigenvalues of \bma{$U$}}. 

%\begin{rem}
%	The quantum versions of the Kraft-McMillan Inequality proved in \cite[Section IIC]{SW01} and \cite[Theorem 3.6]{MR08} are more general than the same proved in \cite[Theorem 1]{BBHZ17}, although the formalisms are quite different in all three. 
%	We quote here the second author's version which is adapted to our formalism, is a generalization of \cite[Theorem 1]{BBHZ17}, but is not quite in the full generality of \cite[Section IIC]{SW01} (in the forward direction) because we only consider uniquely decodable codes (as opposed to the more general notion called \textit{condensable codes} considered in \cite{SW01}). 
%	However, our version does have a converse statement, similar to the classical Kraft-McMillan Inequality, which is missing from the aforementioned quantum versions.
%\end{rem}

The following is an immediate generalization of  \cite[Theorem 2.9]{AW19}, whose proof follows in the exact same manner making the small necessary changes.

\begin{thm}(Quantum Kraft-McMillan Inequality )\label{quantum Kraft}
	Any uniquely decodable quantum code $U$ with length eigenstates over a $d$-ary alphabet must satisfy the inequality $$\tr(U^\dagger d^{-\Lambda}U)\le 1.$$ 
	Conversely, if $U:H_{\mc S}\ra H_{\mc A}^\oplus$ is a linear isometry with length eigenstates satisfying the above inequality, then there exists a c-q scheme $\widetilde U$ with the same number of length $\ell$ eigenstates for each $\ell\in \N$. 
\end{thm}

\DW{The expected length stuff is probably necessary, but may not need to be introduced until the applications section.} 
We would like to find a quantum code which minimizes the amount of resources required. Unfortunately there are numerous ways to define the length of a codeword for an indeterminate-length quantum code (e.g.\ base length \cite{BF02}, exponential length \cite[Definition 6]{BBHZ17}, etc.). 
Here, we follow \cite[Definition 3]{BBHZ17} and define the \textbf{length of a codeword \bma{$|\omega\rangle$}}, which is a normalized vector in $H_{\mc A}^{\oplus}$ given by $|\omega\rangle=U|s\rangle$ for a unique symbol state $|s\rangle\in\{|s_n\rangle\}_{n=1}^N$, as the expectation with respect to the length observable in Equation~\eqref{length observable}. 
Explicitly, the length of a codeword $|\omega\rangle=U|s\rangle$ will be given by a function $\ell: H_{\mc A}^{\oplus}\ra \R^+$, defined as follows: \DW{change this notation to match later notation for the realization morphism}
\begin{equation}\label{q expected length}
	\ell(|\omega\rangle) := \langle \omega |\Lambda|\omega\rangle=
	\langle Us ,\Lambda Us\rangle= \langle s ,U^\dagger \Lambda U s\rangle.
\end{equation}
Whenever $U$ has length eigenstates and is given by Equation~\eqref{length eigenstates}, we see that Equation~\eqref{q expected length} simplifies to 
\begin{equation*}
	\ell(|\omega\rangle) = \sum_{i=1}^d |\langle e_i|s\rangle|^2\ell_i,
\end{equation*}
where $\{\ell_i\}_{i=1}^k$ denotes the set of length eigenvalues of $U$. 

Again we follow \cite{BBHZ17} and, for any ensemble $\mc S=\{p_n,|s_n\rangle\}_{n=1}^N$, we define the \textbf{ensemble state} $\rho_{\mc S}$ of $\mc S$ by 
\begin{equation*}\label{ensemble state}
	\rho_{\mc S}=\sum_{n=1}^N p_n |s_n\rangle\langle s_n|\in S_1(H_{\mc S}).    
\end{equation*} 
If $U$ is a quantum code on $H_{\mc S}$ define the \textbf{average codeword length} with respect to the ensemble $\mc S$ by 
$$EL(U)=\tr(\rho_{\mc S} U^\dagger \Lambda U).$$ 
We denote by $U_{\text{opt}}$ the \textbf{optimal quantum code with length eigenstates} for the ensemble $\mc S$ if 
\begin{equation*}\label{q optimal code}
	\begin{split}
		U_{\text{opt}}:&=\argmin_U \{EL(U) :U \text{ is uniquely decodable with length eigenstates}\}\\
		&=\argmin_U \{EL(U) :\tr(U^\dagger 2^{-\Lambda}U)\le 1\} \\
		&=\argmin_U \{EL(U) :U\text{ is a c-q scheme %with codeword lengths 
			satisfying }\sum_{i=1}^d 2^{-\ell_i}\le 1\} ,
	\end{split}
\end{equation*}
where the second and third equality follow from Theorem~\ref{quantum Kraft}, and the $\{\ell_i\}_{i=1}^d$ in the third equality denote the length eigenvalues of $U$. 
The existence of $U_\opt$ follows from the existence of $C_\opt$ in Equation~\eqref{optimality} by the backward direction of Theorem~\ref{quantum Kraft}. 
The \textbf{optimal average codeword length} for the ensemble $\mc S$ is given by 
\begin{equation}\label{minimum length}
	EL^*(\rho_{\mc S}):= EL(U_\opt)= \tr(\rho_{\mc S} U_\opt^\dagger \Lambda U_\opt).
\end{equation}

\noindent It is shown in \cite[Theorem 2]{BBHZ17} that the optimal c-q scheme (and hence optimal quantum code with length eigenstates by the converse of Theorem~\ref{quantum Kraft}) is given by the classical Huffman codes. The bounds on $EL^*(\rho_{\mc S})$ in terms of the von-Neumann entropy follow immediately. 

\begin{thm}\label{bounds}
	The minimum average codeword length for an ensemble $\mc S$ is bounded as follows, 
	$$ S(\rho_{\mc S})\le EL^*(\rho_{\mc S}) < S(\rho_{\mc S})+1.$$
\end{thm}

\begin{proof}
	See \cite[Theorem 3]{BBHZ17}. 
\end{proof}

Next, we wish to consider the optimal average codeword length per symbol for a collection of ensembles $\{\mc S^k\}_{k=1}^\infty$, where $\mc S^k=\{p(n_1,\cdots, n_k), |s_1s_2\cdots s_k\rangle \}_{n_1,\ldots,n_k=1}^N$ and probabilities given by the pmf $p$ of a stochastic process $\X$. 
We will refer to such collections of ensembles as \textbf{stochastic ensembles}. 
Note that, by the definitions of a stochastic process, a stochastic ensemble $\mc S^k$ must be compatible in the following sense: 
\begin{equation*}\label{compatible}
	\sum_{n_{k+1}=1}^N p(n_1,\cdots,n_{k},n_{k+1})=p(n_1,\cdots, n_{k}),
\end{equation*} 
for all $n_1,\ldots,n_{k}\in\{1,\ldots, N\}\text{ and }k\in\N$.
Notice that we allow for the possibility that preparations of the ensemble at each time be dependent upon previous preparations. If the preparations of the ensemble are independent and identically prepared copies of $\mc S=\{p_n,|s_n\rangle\}_{n=1}^N$; i.e.\ the stochastic process $\X$ is made up of i.i.d.\ copies of a random variable $X$, then $p(n_1,\cdots, n_k)=p_{n_1}p_{n_2}\cdots p_{n_k}$ and $\rho_{\mc S^k}=\rho_{\mc S^1}^{\ten k}$, where 
\begin{equation*}
\rho_{\mc S^k}=\sum_{n_1,\ldots,n_k=1}^N p(n_1,\ldots,n_k)|s_{n_1}\cdots s_{n_k}\ran\lan s_{n_1}\cdots s_{n_k}|. 
\end{equation*}
%, for each $k\in\N$.  
For each $k\in\N$, let 
\begin{equation*}\label{n optimal length}
	EL^*_k(\rho_{\mc S^k})=\frac{1}{k}EL^*(\rho_{\mc S^k})
\end{equation*}
be the \textbf{optimal average codeword length per symbol} for the first $k$ symbols with respect to the ensemble $\mc S^k$, where $EL^*(\rho_{\mc S^k})$ is given by Equation~\eqref{minimum length}. 
Notice that the optimal average codeword length per symbol is defined analogously to the classical case in Equation~\eqref{expected length n}. Then, from Theorem~\ref{bounds}, we have 
\begin{equation}\label{bounds 2}
	\frac{1}{k}S(\rho_{\mc S^k})\le EL^*_k(\rho_{\mc S^k})< \frac{1}{k}S(\rho_{\mc S^k})+\frac{1}{k}.
\end{equation}

\noindent In the following section, we will relate the above quantities to the dynamical entropy of a QMC. 
%Let $\Psi=\{\vp,\mc E_{\gamma,e}^{\Theta}\}\in M_d^{\ten \N}$ be a quantum Markov chain with unique density operator $\rho$ given by $\vp(A)=\tr(\rho A)$ for all $A\in \mc A$. {\color{red} Notice that our notations are starting to overlap.} 




==> singleerror.tex <==
\section{Single qudit error correction}\label{old error}
In what follows, all codings will be done into strings of dits or strings of qudits for classical and quantum codes, respectively. Therefore all codewords will be strings of elements from a $d$-ary alphabet $A$ such that $|A|=d\in\N$ (in the classical case) or, possibly the superposition of, strings from a quantum $d$-ary alphabet, that is a computational basis of dimension $d$. To extend notions of the case of bits, we choose $d=p^m$ for some prime $p$. With this choice of $d$ our alphabet (in the classical case) is taken to be $A=\mathbb{F}_d$, that is the field with $d$ elements. Similarly, in the quantum case our $d$-ary alphabet is
$\mc A=\{|x\ran\,:\,x\in\mathbb{F}_d\}$ which is an orthonormal basis of the Hilbert space $H_{\mc A}=\C^d$. Now we will quickly recall some of the basics of quantum error correction. For a more thorough introduction, see e.g. \cite{fault, goodcodes, gf4, calcliff, nonbinary, ortho,errortheory,mixed,ste98}. 

\subsection{The error group}
Recall that we take pure states of a single qudit system are in $\C^d$ and similarly pure states of an $n$-qudit system are in $\left(\C^d\right)^{\otimes n}\cong\mathbb{C}^{d^n}$. Also, let $d=p^m$ be a power of a prime $p$ and $\mc{A}:=\Big\{|x\ran\,\Big|\,x\in\mathbb{F}_d\Big\}$ be an orthonormal basis for $\mathbb{C}^d$. For sake of calculations we will assume a fixed basis for $\mathbb{F}_d$ over $\mathbb{F}_p$, namely $\{f_i\,:\, i\in\{1,\ldots,m\}\}$.
\begin{defn}
 We define the following unitary operators $X(a)$ and $Z(b)$ for $a,b\in\mathbb{F}_d$ on any $|x\ran\in\mathbb{C}^d$ as
\begin{equation*}
 X(a)|x\ran:=|x+a\ran \;\;\text{ and }\;\; Z(b)|x\ran:=\omega^{b*x}|x\ran,
\end{equation*}
known as the \emph{flip} and \emph{phase} errors respectively, acting on each of the qudits of a code, where $\omega=\text{exp}(2\pi i/p)$ is the primitive $p^\text{th}$ root of unity and \[a*b=\sum_{i=1}^m\alpha_i\beta_i.\] for $a=\sum_{i=1}^m\alpha_if_i$ and $b=\sum_{i=1}^m\beta_if_i$. 
\end{defn}

It is notable that for error groups there is a wonderful connection between our inner product of $a*b$ and $\op{tr}(ab)$ for the standard trace operator  $\mathbb{F}_d\mapsto\mathbb{F}_p$ see \cite{nonbinary}. We make the choice to not use this trace operator only for ease of calculations. Also, we chose to use a notation similar to that in \cite{ortho}.
\begin{rem}
As seen in \cite{nonbinary} this definition is equivalent to first defining $X(\underline{ \;\;\; })$ and $Z(\underline{\;\;\;})$ for parameters in $\mathbb{F}_p$, which act on $\mathbb{C}^p$. Then for $a=\sum_{i=1}^m\alpha_if_i\in\mathbb{F}_d$ we define $X(a)$ and $Z(a)$ on $\mathbb{C}^d\cong\left(\mathbb{C}^p\right)^{\otimes m}$, as \[X(a)=\bigotimes_{i=1}^mX(\alpha_i),\;\;\text{ and }\;\; Z(a)=\bigotimes_{i=1}^mZ(\alpha_i).\]
\end{rem}
\begin{rem}\label{error group}
Notice that for $a,b,c,d\in\mathbb{F}_d$ we have 
\begin{equation*}
\begin{split}
X(a)X(b)&=X(a+b)\\
Z(a)Z(b)&=Z(a+b)\\
Z(b)X(a)&=\omega^{b*a}X(a)Z(b)\\
X(a)Z(b)X(c)Z(d)&=\omega^{b*c-a*d}X(c)Z(d)X(a)Z(b)
\end{split}
\end{equation*}
%Further, if we fix $\{\alpha_i\,:\,i\in\{1,\ldots,t\}\}$ as a basis for the $\mathbb{F}_d$ over $\mathbb{F}_p$, then we need only consider the ``primative" elements $X_i:=X(\alpha_i)$ and for any $k\in\mathbb{F}_p$ \[X^k_i=X(k\alpha_i).\] Therefore the $\big\{X_i\,:\,i\in\{1,\ldots,t\}\big\}$ form a generating set for the multiplicative group of \emph{flip errors} \[\Big\{X(a)\,:\, a\in\mathbb{F}_d\Big\}.\]
%Similarly, if we denote $Z_j:=Z(j)$  for  $j\in\mathbb{F}_p$, the set $\{Z_j\,:\,j\in\mathbb{F}_p\}$ forms a generating set for the mulitplicative group of \emph{phase errors} \[\Big\{Z(b)\,:\,b\in\mathbb{F}_d\Big\}.\]  
\end{rem}


\begin{ex}\label{qubit basis}
For those more familiar with qubits, one quickly notes that when $p=d=2$ then $X$ and $Z$ are exactly the Pauli matrices: 
\[X(0)=Z(0)=\mathbb{1}_2\;\;\;\;X:=X(1)=\begin{bmatrix}0&1\\1&0\end{bmatrix}\;\;\;\;Z:=Z(1)=\begin{bmatrix}1&0\\0&-1\end{bmatrix}\;\;\;\;Y:=iXZ=\begin{bmatrix}0&-i\\i&0\end{bmatrix}\]
\end{ex}



\noindent
Notice, that the set $\mathcal{P}_{\R}:=\{\mathbb{1}_2,X,Y,Z\}$ is linearly independent over both $\C$ or $\R$, and hence span the space of all $2\times 2$ complex matrices. The set $\mathcal{P}_{\R}$ also has the property that the real span (i.e. linearly combinations with all real coefficients) forms all hermitian operators, and that each element of $\mathcal{P}_{\R}$ are themselves hermitian and unitary. Furthermore, the set $\mathcal{P}_{\C}:=\left\{i^\kappa\mathbb{1}_2,\, i^\kappa X, \, i^\kappa Y,\, i^\kappa Z\;\;\Big|\;\; \kappa\in\{0,1,2,3\}\right\}$ form a group with the standard multiplication of matrices. 



%\begin{rem}
%We will often use the standard notation of $X_j$ when the operator $X$ acts on the $j^{\text{th}}$ qudit with the identity acting on the remaining qudits, and similarly for $Z_j$ and $Z_j$. 
%\end{rem}
The following definition is based off those from \cite{nonbinary}.
\begin{defn}
For each $n\in\N$, $\bar{a}:=(a_{1},\ldots,a_{n}),\bar{b}:=(b_{1},\ldots,b_{n})\in\mathbb{F}_d^{n}$, we define
\begin{equation*}
D\left(\bar{a},\bar{b}\right):=X(a_1)Z(b_1)\otimes...\otimes X(a_n)Z(b_n).
\end{equation*}
For $n\in\N$ the collection
\begin{equation*}
\mathcal{E}_n:=\left\{\omega^\kappa D\left(\bar{a},\bar{b}\right)\;\;\Big|\;\; \bar{a},\overline{b}\in\mathbb{F}_d^{n},\,\, \kappa\in\{0,\ldots,p-1\}\,\right\}
\end{equation*}
from Remark \ref{error group} this collection is a group of order $p^{2mn+1}$. We will refer to this group as the \textbf{Error group}.
\end{defn}
It is easily seen that the center, $\mathcal{Z}$, of the group $\mathcal{E}_n$ is generated by $\omega\mathbb{1}$ and therefore has order $p$.
\begin{rem}\label{comm}
For $\overline{a},\overline{b},\overline{c},\overline{d}\in\mathbb{F}_d^n$ and $\kappa,\kappa'\in\{0,\ldots,p-1\}$ then we have the following relations
\begin{equation}\label{eqcomm}
\begin{split}
\left(\omega^\kappa D(\overline{a},\overline{b})\right)\left(\omega^{\kappa'}D(\overline{c},\overline{d})\right)&=\omega^{(\overline{a},\overline{b})\star(\overline{c},\overline{b})}\Big(\omega^{\kappa'}D(\overline{c},\overline{d})\Big)\Big(\omega^\kappa D(\overline{a},\overline{b})\Big)
\end{split}
\end{equation}
where 
\begin{equation}\label{star}
(\overline{a},\overline{b})\star(\overline{c},\overline{d}):=\left\lan\, \overline{b},\overline{c}\,\right\ran-\left\lan\,\overline{a},\overline{d}\,\right\ran\end{equation}
and 
\begin{equation}\label{inner}
\left\lan\,\overline{a},\overline{b}\,\right\ran:=\sum_{i=1}^ta_i*b_i.
\end{equation} 
Therefore, two operators $\omega^\kappa D(\overline{a},\overline{b})$ and $\omega^{\kappa'}D(\overline{c},\overline{d})$ commute if and only if \[(\overline{a},\overline{d})\star(\overline{c},\overline{d})=0.\]
This operation is a symplectic inner product on the space $\mathbb{F}_d^{2n}$. 
\end{rem}



\subsection{Stabilizer Codes}\label{stabilizer}
The objective of quantum stabilizer codes is to be able to protect from any error of a commutative subgroup of errors, $S\subset\mathcal{E}_n$, and correct any error from a large set of errors $\mathscr{E}\subset\mathcal{E}_n$. 
\begin{defn}\label{qsc}
Let $S\subset\mathcal{E}_n$ be a commutative subgroup such that $\mathcal{Z}\subset S$, then we define a \emph{Quantum stabilizer code} as a joint eigenspace of the operators in $S$. 
\DW{Need to be more specific here. Probably include an easy example right after.\RV{what do you mean more specific this is THE definition... I don't see how this doesn't completley define them?}} 
\end{defn}
%\begin{rem}\label{dimQ}
%As $\mathcal{Z}\subset S$ the order of $S$ is a power of $p$ which we will denote as $|S|=p^{r+1}$, then %the joint eigenspaces of $S$ are associated to the $p^r$ linear characters of $S$. \RV{wrong!!!} The %dimension of a quantum stabilizer code, when $p>2$, $Q_{S,\mu}$, for a linear character $\mu$ of $S$ is %$p^{mn-r}$, see \cite{nonbinary}.
%\end{rem}
%A quantum stabilizer code which has the length $n$, that is $Q\subset\mathbb{C}^{d^n}$, and encodes a code from $k$-qudits, i.e. $\op{dim}(Q)=d^k$, then we write that $Q$ is a $[[n,k]]_{d}$ quantum stabilizer code. From Remark \ref{dimQ} we have that for $|S|=p^{r+1}$ a commutative subgroup of $\mathcal{E}_n$ then $Q_{S,\mu}$ is a $[[n,mn-r]]_d$ quantum stabilizer code. Also, from Definition \ref{qsc} it is easily seen that for a commutative subgroup $S\subset\mathcal{E}_n$, we can correct any $E\in S$, and hence correct $|S|$ errors. 



\DW{What types of codes already exist? What do reflexive codes add?} \RV{I think that's more for the introduction}

%we can detect any error $E\in S^\perp\setminus S$, see \cite{nonbinary,ortho}. If we let \[C_S=\{(\overline{a},\overline{b})\,:\,D_{\overline{a},\overline{b}}\in S\}\]and\[C_S^\perp=\{(\overline{a},\overline{b})\in\mathbb{F}_d^{2n}\,:\,(\overline{a}',\overline{b}')\star(\overline{a},\overline{b})=0,\;\forall\, (\overline{a}',\overline{b}')\in C_S\},\] then from Remark \ref{comm} we have, $S^\perp=\{\omega^\kappa D_{\overline{a},\overline{b}}\,:\, (\overline{a},\overline{b})\in C_S^\perp\}$. 

%Thus for $(\overline{a},\overline{b})\in\mathbb{F}_d^{2n}$, defining $\op{wt}(\overline{a},\overline{b})=|\{i\,:\,a_i\neq0\text{ or }b_i\neq0\}|$, then $Q_{S,\mu}$ for a commutative subgroup $S\subset\mathcal{E}$ and a linear character $\mu$, can detect $\op{min}\{\op{wt}(\overline{a},\overline{b})\,:\,(\overline{a},\overline{b})\in C_S^\perp\setminus C_S\}$ errors, see \cite{ortho,nonbinary}. 






==> toric.tex <==
\section{Classical Toric Codes}
Toric codes are evaluation codes which arise from the global sections of a certain divisor $D$ of a smooth toric variety $X$ over a finite field $K:=\mathbb{F}_d$ where $d$ is a prime power, i.e. $X\subseteq(K)^N$ for some $N\in\N$. Let $S\subseteq T\cong (K^*)^N$ with $|S|=n$, then for every $t\in T$ we evaluate the rational functions in $H^0\left(X,O_X(D)\right)$ by
\begin{equation*}
\begin{split}
H^0\left(X,O_X(D)\right)&\mapsto K\\
f&\mapsto f(t).
\end{split}
\end{equation*}
Let $H^0\left(X,O_X(D)\right)^{\text{Frob}}$ denote the rational functions in $H^0\left(X,O_X(D)\right)$ that are invariant under the action of the Frobenius. Evaluating at all points in $S$, we obtain the toric code associated to $X$ and $S$, which we will denote $C_{X,S}\subset K^{n}$.

\begin{ex}[\textbf{Reed-Solomon Codes $N=1$}]
Let $x_1,x_2,\ldots,x_n\in K$ be $n$ distinct elements and let $0<m\leq n$.

To the word $(a_0,a_1,\ldots,a_{m-1})\in K^m$ of length $m$ we associate the polynomial
\[f(Y)=a_0+a_1Y+\ldots +a_{m-1}Y^{m-1}\in K[Y]\]
and upon evaluetion the Reed-Solomon code word 
\[\Big(f(x_1),f(x_2),\ldots,f(x_n)\Big)\in K^n\]
The Reed-Solomon code $C_{n,m}\subseteq K^n$ is the subspace of all Reed-Solomon code words coming from all polynomials $f(Y)\in K[Y]$ with $\text{deg}\Big(f(Y)\Big)<m\leq n$.

It is well Known that the Reed-Solomon code $C_{n,m}\subseteq K^n$ has dimension $\text{dim}_K(C_{n,m})=m$, minimum distance $d(C_{n,m})=n-m+1$ and corrects at most $\frac{d(C_{n,m})}{2}$ errors. 
\end{ex}

\subsection{Integral Convex Polytopes}
Toric varieties and thus toric codes correspond to integral convex polytopes in $\mathbb{R}^r$ for some $r\in\N$, i.e. a compact convex polyhedron such that the vertices belong to $\mathbb{Z}^r$. Let $\Box$ be an integral convex polytope, then for each vertex $\vec{a}=(a_1,\ldots,a_r)\in\mathbb{Z}^r$ we can associate a monomial 
\begin{equation*}x^{\vec{a}}:=\prod_{i=1}^rx_i^{a_i}\in K[x_1,\ldots,x_r]\end{equation*}





\section{Quantum Toric Codes}

\section{Toric approach to indeterminate length codes}
